Competing instabilities in quench experiments with ultracold Fermi gases near a Feshbach resonance

Tunability of effective two body interactions near Feshbach resonances is a powerful experimental tool in systems of ultracold atoms. It has been used to explore a variety of intriguing phenomena in recent experiments. However not all of the many-body properties of such systems can be understood in terms of effective models with contact interaction given by the scattering length of the two particles in vacuum. For example, when a two component Fermi mixture is quenched to the BEC side of the Feshbach resonance, a positive scattering length suggests that interactions are repulsive and thus collective dynamics should be dominated by the Stoner instability toward a spin polarized ferromagnetic state. On the other hand, existence of low energy two particle bound states suggests a competing instability driven by molecule formation. Compe- tition between spontaneous magnetization and pair formation is determined by the the interplay of two-particle and many-body phenomena. In these lecture notes we summarize our recent theoretical results, which analyzed this competition from the point of view of unstable collective modes. We also comment on the relevance of this theoretical analysis to recent experiments reported in Ref. (Jo, Lee, Choi, Christensen, Kim, Thywissen, Pritchard and Ketterle, 2009).

==> tex2bib <==
#! /usr/local/bin/perl 

$Script = 'tex2bib'; 
$Version=0.97;  # 22 Feb 2006 10:50:35
$Author='Michael Friendly (friendly@yorku.ca)';

# Copyright (c) 1997 Michael Friendly
#
# License:
#  This is free software subject to copyright, released according to the
#  BSD style license.  It may be freely used, modified and distributed.
#  See: http://www.ctan.org/tex-archive/help/Catalogue/licenses.bsd.html
#  for details and further information.

# tex2bib
#   Input a TeX document containing \bibitems, translate these
#   to BibTeX format
#
# Usage:
#		tex2bib [-k][-i infile] [-o outfile]
#		-k:  regenerate keys
#		if infile not given, reads from stdin
#		if outfile not given, prints to stdout

# The entire tex document is scanned for \bibitems, ending when
# the string '\end{thebibliography}' is read.

# Assumes that bibitems are formatted as follows:
#  -- {key}author(s), (date) at the beginning
#  -- titles of books or names of journals: {\em title}
#  -- article titles: 	after date, `` '' quotes optional
#  -- volume, pages: 	{\it vol}, nnn-nnn.
#  -- publisher/address:    address:publisher
#
#  All text in the bibitem which cannot be parsed is included
#  in a note = { } field
#
# Changes
#  0.96 1998/06/22  Allow \bibitem keys to contain [\w:-]
#  0.97 2006/02/21  Added BSD license
#################################################################
# Examples of a book, article, inproceedings:

#\bibitem{Bertin83}Bertin, J. (1983),
#        {\em Semiology of Graphics} (trans. W. Berg).  Madison, WI:
#        University of Wisconsin Press.
#
#\bibitem{Bickel75}Bickel, P. J., Hammel, J. W. and O'Connell, J. W.
#        (1975).
#        Sex bias in graduate admissions: data from Berkeley.  {\em
#        Science}, {\it 187}, 398-403.
#
#\bibitem{Farebrother87}Farebrother, R. W. (1987),
#        ``Mechanical representations of the ${L}_1$ and ${L}_2$ estimation
#        problems'', In Y. Dodge (ed.)  {\em Statistical data analysis
#        based on the L1 norm and related methods}, Amsterdam:
#        North-Holland., 455-464.


# These are output as:

#@Book{  Bertin:83,
#    author      = {J. Bertin},
#    year        = 1983,
#    title       = {Semiology of Graphics},
#    publisher   = {University of Wisconsin Press},
#    address     = {Madison, WI},
#    note        = {(trans. W. Berg).}
#}
#@Article{       Bickel:75,
#    author      = {Bickel, P. J. and Hammel, J. W. and O'Connell, J. W.},
#    year        = 1975,
#    title       = {Sex Bias in Graduate Admissions: Data from Berkeley},
#    journal     = {Science},
#    volume      = 187,
#    pages       = {398-403}
#}
#@InCollection{  Farebrother:87,
#    author      = {R. W. Farebrother},
#    year        = 1987,
#    title       = {Mechanical Representations of the ${L}_1$ and ${L}_2$ Estimation Problems},
#    booktitle   = {Statistical Data Analysis Based on the L1 Norm and Related Methods},
#    editor      = {Y. Dodge},
#    publisher   = {North-Holland},
#    address     = {Amsterdam},
#    pages       = {455-464}

# Text in a bibitem is removed from the bibitem as it is assigned to
# bibtex fields.  Any text remaining is assigned to a note={  } field
# at the end.  Since the parsing is heuristic, some manual fixup work
# can be expected at the end.

#################################################################

require 'getopt.pl' ;

    Getopt("oikdrt:");             # ARGV now contains [inputfile] and
                                #   $opt_o, $opt_i might be set.
	
	$default_type = $opt_t || 'Article';
	
    open(STDIN, "<$opt_i") or die "-i $opt_i: can't open.\n" if $opt_i ;
    open(STDOUT, ">$opt_o") or die "-o $opt_o: can't create.\n" if $opt_o ;

#######################  Process input files  ####################
$bibs=0;
while (<>)
{
	/^\s*\\end\{thebibliography/ && last;
	if (/\\bibitem\s*\{([\w\d:-]+)\}/) {
		$bibs++;
		$key = $1;
#		print STDERR "$bibs key: $key\n";
	}
	# skip if we're still reading tex text (no bibitems encountered)
	next unless $bibs;
	chomp;
	s/^\s*/ /;
	$lines .= $_;
}

# All lines containing \bibitems have been read into the $lines string.
# Now, split into separate items

@items = split(/\\bibitem\s*/, $lines);
print STDERR "items has ", scalar(@items), " items\n";

@months = qw(january february march april may jun july august september
	october november december);
$month_pat = join('|', @months);

foreach (@months) {
	$month_abbrv{$_} = substr($_, 0,3);
}
	
$ordinal = 'first|second|third|fourth|1st\.?|2nd\.?|3rd\.?|4th\.?';

# title words to ignore for casing;
foreach ( qw(a about an and by for from in of on the to von with) ) {
	$ignore_case{$_} = 1;
}

$outitems =0;
%keys_seen = {};

foreach $i (0..$#items) {
	undef $title;
	undef $pages;
	undef $journal;
	undef $volume;
	undef $number;
	undef $booktitle;
	undef $editor;
	undef $edition;
	undef $month;
	undef $publisher;
	undef $address;
	undef $chapter;
	undef $rest;
	
	print "$items[$i]\n" if $opt_d;
	# assume each entry starts with
	#	{key}Author, F.I. etc (date[a-z]?)
#	$items[$i] =~ /^\{([^}]+)\}([^\(]*)\((\d{4})[a-z]?\)[,.]?\s*/;
#	($key, $authors, $date) = ($1, $2, $3);
	$items[$i] =~ /^\{([^}]+)\}\s*/;
	$key = $1;
#	print  "key: $key\n";
	$rest = $';
		
	$rest =~ /\((\d{4})[a-z]?\)[,.]?\s*/ &&
		do {
			$authors = $`;
			$date = $1;
			$rest = $';
		};

	unless (defined($key)) {
		print STDERR "Skipping: $authors, $date in \n$items[$i]\n";
		next;
	}
		

	$rest =~ s/^[.,]?\s+//;
	$rest =~ s/\s+$//;

#	print "key: $key\n";
#	$key =~ m/(['A-Za-z]+)([^:]*)/ &&
#		do { $key = "$1:$2"; };
#	print "key: $key\n";
			
	&parse_authors;

	$orig_key = $key;
	$key = &generate_key if $opt_k or $keys_seen{$key};
	
	# if the $key has already been seen, make a new, unique one
	if ($keys_seen{$key}) {
		foreach $suffix (('b'..'z')) {
			$try = $key . $suffix;
#			print STDERR "Seen $key ... trying $try\n";
			unless ($keys_seen{$try}) {$key = $try; last; };
		}
		print STDERR "New unique key generated: $key (was $orig_key)\n"
			unless $key eq $orig_key;
	}
	$keys_seen{$key}++;
	
	# assume it's an article at first
	$type = '@' . $default_type;

	if ($rest =~ /^\{\\em\s+/) {
	#tech report or book
		$type = '@Book';
		$rest =~ m/^\{\\em\s+(['\w ,?:]+)\}[., ]*/;
		$title = $1;
		$rest = $';
		&parse_edition;
		&parse_publish;

		$rest =~ m/\sreport(s?)[,]?\s*/i &&
			do {
				$type ='@TechReport';
				$rest = $` . $';
				&parse_report_number;
			};
	}

	else {
		#does it begin with quoted title?
		if ($rest =~ /^``/){
			$rest =~ m/^``([^`]+)''[., ]*/;
			$title = $1;
			$rest = $';
		}
		else {
			$rest =~ m#^(['\{\}\w\d,\(\)\\ :\?/-]+)[. ]*#;
			$title = $1;
			$rest = $';
		}
		$rest =~ s/^[,\s]+//;
		
		if ($rest =~ /^\{\\em\s+/) {
			$rest =~ m/^\{\\em\s+([\w\\& ,'-?]+)\}[., ]*/;
			$journal = $1;
			$rest = $';
		}
		# parse {\it volume (number)}
		&parse_volume;
			
		$rest =~ m/,?\s*(\d{1,4}--?\d{1,4})[.,]?\s*/ && 
			do {
			$pages = $1;
			$rest = $`. $';
			$pages =~ s/(\d)-(\d)/$1--$2/;
			};

		$rest =~ m/\(($month_pat)\)/i &&
			do {
				($month = $1) =~ tr/A-Z/a-z/;
				$month = $month_abbrv{$month};
				$rest = $` . $';
			};
			
		$rest =~ m/(technical|tech\.)\s+report[,.]?/i &&
			do {
				$type ='@TechReport';
				$rest = $` . $';
				&parse_report_number;
			};
		
		$rest =~ m/^In\s+/i &&
			do {
				$rest = $';
				$type ='@InCollection';  # maybe, proceedings
				$rest =~ m/\{\\em\s+([\w ,':!?]+)\}[., ]*/ &&
					do {
					$booktitle = $1;
					$rest = $` . $';
					$type = '@InProceedings' if $booktitle =~ m/proceedings/i;
					};
				$rest =~ m/([\w., ]+)\s+\(eds?\.\)[,.]?\s*/i &&
					do {
					$editor = $1;
					$rest = $` . $';
					};
				$rest =~ m/Chapter\s+(\d+)[.,]?\s*/i &&
					do {
					$chapter = $1;
					$rest = $` . $';
					};
				
				&parse_edition;
				&parse_publish;
			};

		$rest =~ m/proceedings/i &&
			do {
				$type = '@InProceedings';
#	print "$items[$i]\n";
			};
	}

	$rest =~ s/^\s+//;
	$rest =~ s/$date([,]?)//;
	
	$title = &case_title($title);
	$booktitle = &case_title($booktitle) if $booktitle;
	
	print "$type\{$key";
	print ",\n    author\t= {$authors}";
	print ",\n    year\t= $date";
	print ",\n    title\t= {$title}" if $title;
	print ",\n    booktitle\t= {$booktitle}" if $booktitle;
	print ",\n    edition\t= {$edition}" if $edition;
	print ",\n    editor\t= {$editor}" if $editor;
	print ",\n    publisher\t= {$publisher}" if $publisher;
	print ",\n    address\t= {$address}" if $address;
	print ",\n    journal\t= {$journal}" if $journal;
	print ",\n    volume\t= $volume" if $volume;
	print ",\n    month\t= $month" if $month;
	print ",\n    number\t= $number" if $number;
	print ",\n    pages\t= {$pages}" if $pages;
	print ",\n    chapter\t= {$chapter}" if $chapter;
	print ",\n    note\t= {$rest}" if $rest;
	print "\n\}\n";
	$outitems++;	
}
print STDERR "$outitems items processed\n";
exit;

########################### subroutines #############################

# separate multiple authors with 'and'
sub parse_authors {
	# fix authors field
	$authors =~ s/\s+$//;
	$authors =~ s/\\&/and/;
	$authors =~ s/([A-Z])\.([A-Z])\./$1. $2./g;
	$authors =~ s/ ([A-Z])\.,\s+(?!Jr.)/ $1. and /g;
	$authors =~ s/ and and / and /;
#	$authors =~ s/Friendly, M./Friendly, Michael/;
	$authors =~ s/M. Friendly/Friendly, M./;
	local($commas) = ($authors =~ tr/,/,/);
	if ($opt_r && $commas == 1) {
		@auth = split(/, /, $authors);
		$authors = join(' ',reverse(@auth));
	}

}

# extract last names of authors into @auth array
sub split_authors {
	@auth = split(/ and /, $authors);
	@auth =~ grep(s/, .*$//g,@auth);          # strip trailing initials
	@auth =~ grep(s/^([A-Z]\.\s*)+//g,@auth);
#	@auth =~ grep(s/^[a-z ]+//,@auth);        # strip any name prefixes

	foreach  $i (0..$#auth) {
		@n = split(/ /, $auth[$i]);
		$auth[$i] = pop(@n);               # strip anything before lastname
		$auth[$i] =~ s/[^\w]//g;           # remove non-word chars 		
	}
		
#	print STDERR "Authors: $authors --> ", 
		join('|',@auth),"\n"    if scalar(@auth) > 1;
		
}

sub parse_volume {
	$rest =~ m/,?\s*\{\\it\s+([A-Za-z \d()]+)\s*\}[.,]?/ &&
		do {
		$volume = $1;
		$rest = $`. $';
		$volume =~ m/\(([ \w]+)\)/ &&
			do {
				$volume = $`;
				$number = $1;
			};
		$volume = "{$volume}" unless $volume =~ m/^\d*$/;
		$number = "\{$number\}" unless $number =~ m/^\d*$/;
		};
			
}

# find publisher and address in book/inproceedings items
#	assume the format is address:publisher
sub parse_publish {
	local($before, $after);
	$rest =~ m#:\s*([\w-\\/& ]+)[.]?# &&
		do {
			$publisher = $1;
			($before, $after) = ($`, $');
			$before =~ m/([\w, ]+)$/ &&
				do {
				$address = $1;
				$before = $`;
				$address =~ s/^\s+//;
				};
			$rest = $before . $after;
		};
}

sub parse_report_number {
	$rest =~ m/\s*(no\.|number)\s+(\d+)[,.]?\s*/i &&
		do {
		$number = $2;
		$rest = $` . $';
		}
}

sub parse_edition {
	$rest =~ m/\(?($ordinal).*(edition|ed\.)\)?\.?\s*/i &&
		do {
		$edition = $1;
		$rest = $` . $';
		}
}

# Initial-caps for all non-ignored words
sub case_title {
	local($t) = @_;
	local(@words) = split(/\s+/, $t);
	local($w) =0;
	local($colon);
	foreach (@words) {
		$w++;
		next if /^[A-Z]/;
		unless ($colon) {next if $ignore_case{$_}};		
		s/^([a-z])/\u$1/;
		$colon = tr/:/:/;
	}
	join(' ', @words);
}

sub generate_key {
	local($yr, $key);
	($yr = $date) =~ s/^1\d//;
	&split_authors;	
	if (scalar(@auth) < 3) {
		$key = join('', @auth, ':', $yr);
	}
	else {
		$key = join('', $auth[0], '-etal:', $yr);
	}
#	print STDERR "New key: $key (", join('|', @auth), ": $date)\n";
	$key;
}

